Delivery Time Minimization in Edge Caching: Synergistic Benefits of Subspace Alignment and Zero Forcing

An emerging trend of next generation communication systems is to provide network edges with additional capabilities such as additional storage resources in the form of caches to reduce file delivery latency. To investigate this aspect, we study the fundamental limits of a cache-aided wireless network consisting of one central base station, $M$ transceivers and $K$ receivers from a latency-centric perspective. We use the normalized delivery time (NDT) to capture the per-bit latency for the worst-case file request pattern at high signal-to-noise ratios (SNR), normalized with respect to a reference interference-free system with unlimited transceiver cache capabilities. For various special cases with $M=\{1,2\}$ and $K=\{1,2,3\}$ that satisfy $M+K\leq 4$, we establish the optimal tradeoff between cache storage and latency. This is facilitated through establishing a novel converse (for arbitrary $M$ and $K$) and an achievability scheme on the NDT. Our achievability scheme is a synergistic combination of multicasting, zero-forcing beamforming and interference alignment.

==> arxiv/tikz_stuff.tex <==
\usetikzlibrary{decorations.text}
\usepgfplotslibrary{fillbetween}
\usetikzlibrary{calc, fit}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{patterns}

\newcommand{\SymMod}[0]{
	\begin{tikzpicture}[
	roundnode/.style={circle, draw=green!60, fill=green!5, very thick, minimum size=7mm},
	squarednode/.style={rectangle, draw=red!60, fill=red!5, very thick, minimum size=5mm},
	]
	\node[squarednode] (eNB) at (0.0, 2.6+2) {DeNB};
	\node[squarednode] (HeNB) at (2+1, 0.6+2) {RN$_1$};
	\node[squarednode] (Utwo) at (3.75+3, 2.6+2) {UE$_1$};
	
	\draw[->, black, thick] (0.6, 2.6+2) -- (3.3+3, 2.6+2) node[pos=0.5,sloped,above] {$g_{1}$};
	\draw[->, thick, blue] (0.6, 2.6+2) -- (1.5+1, 0.6+2) node[pos=0.5,sloped,above] {$f_1$};
	\draw[->, magenta, thick] (2.45+1, 0.6+2) -- (3.25+3, 2.5+2) node[pos=0.5,sloped,below] {$h_{11}$};
	
	\node (ch) at (2+1, 0+2) {\includegraphics[scale=.3]{content/cache.pdf}};
	\draw[<->] (2.3+1, -0.23+2) -- (2.3+1, 0.24+2) node[pos=0.5,sloped, below] {$\scriptstyle\mu NL$};
	
	\node[squarednode] at (2+1, 0) {RN$_M$};
	\node[squarednode] at (3.75+3, 0) {UE$_K$};
	
	\node (ch) at (2+1, -0.6)
	{\includegraphics[scale=.3]{content/cache.pdf}};
	\draw[<->] (2.3+1, -0.23-0.6) -- (2.3+1, 0.24-0.6) node[pos=0.5,sloped, below] {$\scriptstyle\mu NL$};
	
	\draw[->, black, thick] (0.6, 2.6+2) to [out=-10, in=-230] (3.25+3, 0);
	\node at (3.45, 3.6) {$g_{K}$};
	\draw[->, thick, blue] (0.6, 2.6+2) -- (1.4+1, 0) node[pos=0.5,sloped,above] {$f_M$};
	\draw[->, magenta, thick] (2.45+1, 0.6+2) -- (3.25+3, 0) node[pos=0.5,sloped,below] {$h_{K1}$};
	\draw[->, magenta, thick] (2.5+1, 0) -- (3.25+3, 2.5+2) node[pos=0.5,sloped,below] {$h_{1M}$};
	\draw[->, magenta, thick] (2.5+1, 0) -- (3.25+3, 0) node[pos=0.5,sloped,below] {$h_{KM}$};
	
	\path (3.75+3, 2.6+2) -- (3.75+3, 0) node [black, scale=3.0, midway, sloped] {$\dots$};
	\path (2+1, 0.24+2) -- (2+1, 0) node [black, scale=1.5, midway, sloped] {$\dots$};
	\end{tikzpicture}
}

\newcommand{\PlotNDTMOneKOne}[0]{
		\begin{axis}[
			axis x line=bottom, axis y line=left,
			ymin=0, ymax=3, ytick={1,...,2}, ylabel={\small Normalized Delivery Time},
			xmin=0, xmax=1.2, xtick={1,...,1.2}, xlabel=$\mu$, grid=major
			]
			
			\addplot+[name path=f1, no markers, decoration={
			%	text along path,
				text={}, raise=1ex,
				text align={center}
			}, postaction={decorate}, very thick, blue, domain=0:1, smooth]{2-x};
			\addplot[very thick, blue, domain=1:1.2, smooth]{1};
			
			\path[name path=axis] (axis cs:0,3) -- (axis cs:0,2) -- (axis cs:1,1) -- (axis cs:1.2,1) -- (axis cs:1.2,3) -- (axis cs:0,3);
			\addplot[blue!10] fill between[of=axis and f1];
			\addplot[red, mark=otimes*, mark size=3.75pt, only marks] coordinates {(0,2) (1,1)};
		\end{axis}
}

\newcommand{\PlotNDTMOneKTwo}[0]{
	\begin{axis}[
	axis x line=bottom, axis y line=left,
	ymin=0, ymax=4, ytick={1,3}, ylabel={\small Normalized Delivery Time},
	xmin=0, xmax=1.2, xtick={1}, xlabel=$\mu$, grid=major,
	]
	
	\addplot+[name path=f1, no markers, decoration={
	%	text along path,
		text={}, raise=1ex,
		text align={center}
	}, postaction={decorate}, very thick, blue, domain=0:1, smooth]{3-x-x};
	\addplot[very thick, blue, domain=1:1.2, smooth]{1};
	
	\path[name path=axis] (axis cs:0,4) -- (axis cs:0,3) -- (axis cs:1,1) -- (axis cs:1.2,1) -- (axis cs:1.2,4) -- (axis cs:0,4);
	\addplot[blue!10] fill between[of=axis and f1];
	\addplot[red, mark=otimes*, mark size=3.75pt, only marks] coordinates {(0,3) (1,1)};
	\end{axis}
}

\newcommand{\PlotNDTMOneKGreatTwo}[0]{
	\begin{axis}[
	axis x line=bottom, 
	axis y line=left,
	ymin=0, 
	ymax=5, 
	ytick={1.5,1.6,2.5, 4}, 
	ylabel={\small Normalized Delivery Time},
	xmin=0, 
	xmax=1.2, 
	xtick={0.5, 0.8,1}, 
	xlabel=$\mu$, 
	xticklabels={$\nicefrac{1}{2}$,$\mu_1=\frac{K+1}{2K-1}$,$1$},
	yticklabels={$\ $,$\ $,$\frac{K+2}{2}$, \scriptsize{$K+1$}}, 
%	yticklabel style={rotate=90}, 
	grid=major, 
	]
	
	\addplot+[name path=f1, no markers, decoration={
		text along path,
		text={}, raise=1ex,
		text align={center}
	}, postaction={decorate}, very thick, blue, domain=0:0.8, smooth]{4-x-x-x};
		\addplot+[no markers, decoration={
			%text along path,
			text={}, raise=1ex,
			text align={center}
		}, postaction={decorate}, very thick, blue, domain=0.8:1, smooth] plot coordinates {
		(0.8,1.6)
		(1,1.5)
	};
	
	\addplot+[no markers, decoration={
				%text along path,
				text={}, raise=1ex,
				text align={center}
			}, postaction={decorate}, red, dashed, domain=0:1, smooth] plot coordinates {
			(0,4)
			(1,1.5)
	};
		
	\addplot[blue, very thick, domain=1:1.2, smooth]{1.5};
	
	\path[name path=axis1] (axis cs:0,5) -- (axis cs:0,4) -- (axis cs:0.8,1.6) -- (axis cs:1,1.5) -- (axis cs:1.2,1.5) -- (axis cs:1.2,5) -- (axis cs:0,5);
	\addplot[blue!10] fill between[of=axis1 and f1];
	\addplot[red, mark=otimes*, mark size=3pt, only marks] coordinates {(0,4) (0.8, 1.6) (1,1.5)};
	\addplot[blue, mark=square*, mark size=3pt, only marks] coordinates {(0.5, 2.5)};
	\draw [dashed] (axis cs:0.8,1.6) -- (axis cs:0.8,5);
	\draw[->] (axis cs:0.8,4) -- node [text width=2.0cm,above] {$\:\:\:\text{DoF}_{\Sigma}<2$}(axis cs:0.5,4);
	\draw[->,red!100] (axis cs:0.8,4) -- node [text width=2.0cm,above] {$\:\:\:\:\text{DoF}_{\Sigma}=2$}(axis cs:1.1,4);	
	\end{axis}
	\node at (-.3,1.4) {$\frac{K}{2}$};
	\node at (-.5,2.0) {$\frac{K^2-1}{2K-1}$};
}

\newcommand{\PlotNDTMTwoKOne}[0]{
	\begin{axis}[
		axis x line=bottom, axis y line=left,
		ymin=0, ymax=4, ytick={1,3}, ylabel={\small Normalized Delivery Time},
		xmin=0, xmax=1.2, xtick={0.5,1}, xlabel=$\mu$, grid=major, 	xticklabels={$\nicefrac{1}{2}$,$1$}
		]
		
		\addplot+[name path=f1, no markers, decoration={
			%	text along path,
			text={}, raise=1ex,
			text align={center}
		}, postaction={decorate}, very thick, blue, domain=0:0.5, smooth]{3-4*x};
		\addplot[very thick, blue, domain=0.5:1.2, smooth]{1};
		
		\path[name path=axis] (axis cs:0,4) -- (axis cs:0,3) -- (axis cs:0.5,1) -- (axis cs:1.2,1) -- (axis cs:1.2,4) -- (axis cs:0,4);
		\addplot[blue!10] fill between[of=axis and f1];
		\addplot[red, mark=otimes*, mark size=3.75pt, only marks] coordinates {(0,3) (0.5,1)};
	\end{axis}
}

\newcommand{\PlotNDTMTwoKTwo}[0]{
	\begin{axis}[
		axis x line=bottom, axis y line=left,
		ymin=0, ymax=5, ytick={1,4}, ylabel={\small Normalized Delivery Time},
		xmin=0, xmax=1.2, xtick={0.4444444444444, 0.5, 1}, xlabel=$\mu$, grid=major, 	xticklabels={$\frac{4}{9}$,$\frac{1}{2}$, $1$}, extra y ticks={1.33333333333333, 1.25}, extra y tick labels={$\quad\frac{4}{3}$,$\frac{5}{4}$}, extra y tick style={y tick label style={rotate=90}},
		]
		
		\addplot+[name path=f1, no markers, decoration={
			%	text along path,
			text={}, raise=1ex,
			text align={center}
		}, postaction={decorate}, very thick, blue, domain=0:4/9, smooth]{4-6*x};
		
		\addplot+[name path=f2, no markers, decoration={
					%	text along path,
			text={}, raise=1ex,
			text align={center}
			}, postaction={decorate}, very thick, blue, domain=4/9:0.5, smooth]{2-1.5*x};
		
		\addplot+[name path=f3, no markers, decoration={
			%	text along path,
			text={}, raise=1ex,
			text align={center}
			}, postaction={decorate}, very thick, blue, domain=0.5:1, smooth]{1.5-0.5*x};
			
		\addplot[very thick, blue, domain=1:1.2, smooth]{1};
		
		\path[name path=axis] (axis cs:0,5) -- (axis cs:0,4) -- (axis cs:4/9,4/3) -- (axis cs:0.5,5/4) -- (axis cs:1,1) -- (axis cs:1.2,1) -- (axis cs:1.2,5) -- (axis cs:0,5);
		\addplot[blue!10] fill between[of=axis and f1];
		\addplot[red, mark=otimes*, mark size=3.75pt, only marks] coordinates {(0,4) (4/9,4/3) (0.5,5/4) (1,1)};
	\end{axis}
}

\newcommand{\FilesKThree}[0]{
	\centering
\begin{tabular}{c|ccccc}
\multicolumn{1}{c}{} & \multicolumn{4}{c}{\textcolor{red}{RN \& DeNB}} & \textcolor{blue}{DeNB only}\\   
File $W_1$ & \tikz[remember picture]{\node[anchor=base,inner sep=0pt] (a1) {\textcolor{OliveGreen}{$\eta_{1,1}$}};} & \textcolor{OliveGreen}{$\eta_{1,2}$} & \textcolor{OliveGreen}{$\eta_{1,3}$} & $\eta_{1,4}$ & \tikz[remember picture]{\node[anchor=base,inner sep=0pt] (a5) {$\eta_{1,5}$};} \\
File $W_2$ & \textcolor{OliveGreen}{$\eta_{2,1}$} & \textcolor{OliveGreen}{$\eta_{2,2}$} & \textcolor{OliveGreen}{$\eta_{2,3}$} & $\eta_{2,4}$ & $\eta_{2,5}$ \\
File $W_3$ & \textcolor{OliveGreen}{$\eta_{3,1}$} & \textcolor{OliveGreen}{$\eta_{3,2}$} & \textcolor{OliveGreen}{$\eta_{3,3}$} & $\eta_{3,4}$ & $\eta_{3,5}$ \\
File $W_4$ & $\eta_{4,1}$ & $\eta_{4,2}$ & $\eta_{4,3}$ & \tikz[remember picture]{\node[anchor=base,inner sep=0pt] (d4) {$\eta_{4,4}$};} & \tikz[remember picture]{\node[anchor=base,inner sep=0pt](d5) {$\eta_{4,5}$};}\\ [0.5\baselineskip] \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textcolor{OliveGreen}{ZF symbols}}
\tikz[remember picture,overlay]{
\node [draw = red, fit = (a1) (d4)] {};
}
\tikz[remember picture,overlay]{
	\node [draw = blue, fit = (a5) (d5)] {};
}
\end{tabular}
}

\newcommand{\ZFKThree}[0]{
	\centering
	\begin{tabular}{c|ccc}
		 & \multicolumn{3}{c}{ZF map}\\ \hline 
		UE$_1$ &  \textcolor{OliveGreen}{$\eta_{2,1}$} & \textcolor{OliveGreen}{$\eta_{2,2}$} & \textcolor{OliveGreen}{$\eta_{3,3}$} \\ \hline 
		UE$_2$ & \textcolor{OliveGreen}{$\eta_{3,1}$} & \textcolor{OliveGreen}{$\eta_{3,2}$} & \textcolor{OliveGreen}{$\eta_{1,3}$} \\ \hline 
		UE$_3$ & \textcolor{OliveGreen}{$\eta_{1,1}$} & \textcolor{OliveGreen}{$\eta_{1,2}$} & \textcolor{OliveGreen}{$\eta_{2,3}$} \\ \hline
	\end{tabular}
}

\newcommand{\AlignGraph}[0]{
	
	% Draw Layers
	\draw[fill=blue!20,draw=white] (-3.5,-0.5) rectangle (-0.5,5.5);
	\draw[fill=green!20,draw=white] (4.5,-0.5) rectangle (-0.5,5.5);
	\draw[fill=magenta!20,draw=white] (4.5,-0.5) rectangle (10,5.5);
	
	% Draw Curly Braces per Layer
	\draw [thick,decoration={brace,raise=0.1cm
	},decorate] (-3.5,5.5) -- (-0.5,5.5) 
	node [pos=0.5,anchor=north,yshift=1.15cm,align=left] {\small \textcolor{blue}{Layer 1}: Align 2 \\\small symbols per UE};
	\draw [thick,decoration={brace,raise=0.1cm
	},decorate] (-0.5,5.5) -- (4.5,5.5) 
	node [pos=0.5,anchor=north,yshift=1.15cm,align=left] {\small \textcolor{OliveGreen}{Layer 2}: Align 3 \\\small symbols per UE};
	\draw [thick,decoration={brace,raise=0.1cm
	},decorate] (4.5,5.5) -- (10,5.5) 
	node [pos=0.5,anchor=north,yshift=1.15cm,align=left] {\small \textcolor{magenta}{Layer 3}: Align 3 \\\small symbols per UE};
	
%	\begin{scope}[every node/.style={circle,thick,draw}]
%		\node (d5) at (-3,2.5) {\footnotesize $d_5$};
%		\node (b4) at (-0.5,0) {\footnotesize $b_4$};
%		\node (b2) at (2.0,0) {\footnotesize $b_2$};
%		\node (a5) at (4.5,0) {\footnotesize $a_5$};
%		\node (a1) at (7.0,0) {\footnotesize $a_1$};
%		\node (c3) at (9.5,0) {\footnotesize $c_3$};		
%		\node (c4) at (-0.5,2.5) {\footnotesize $c_4$};
%		\node (c2) at (2.0,2.5) {\footnotesize $c_2$};
%		\node (b5) at (4.5,2.5) {\footnotesize $b_5$};
%		\node (b1) at (7.0,2.5) {\footnotesize $b_1$};
%		\node (a3) at (9.5,2.5) {\footnotesize $a_3$};		
%		\node (a4) at (-0.5,5) {\footnotesize $a_4$};
%		\node (a2) at (2.0,5) {\footnotesize $a_2$};
%		\node (c5) at (4.5,5) {\footnotesize $c_5$};
%		\node (c1) at (7.0,5) {\footnotesize $c_1$};
%		\node (b3) at (9.5,5) {\footnotesize $b_3$};
%	\end{scope}

	\begin{scope}[every node/.style={circle,thick,draw}]
			\node (d5) at (-3,2.5) {\footnotesize $\eta_{4,5}$};
			\node (c4) at (-0.5,0) {\footnotesize $\eta_{3,4}$};
			\node (c2) at (2.0,0) {\footnotesize $\eta_{3,2}$};
			\node (b5) at (4.5,0) {\footnotesize $\eta_{2,5}$};
			\node (a3) at (7.0,0) {\footnotesize $\eta_{1,3}$};
			\node (b1) at (9.5,0) {\footnotesize $\eta_{2,1}$};		
			\node (b4) at (-0.5,2.5) {\footnotesize $\eta_{2,4}$};
			\node (b2) at (2.0,2.5) {\footnotesize $\eta_{2,2}$};
			\node (a5) at (4.5,2.5) {\footnotesize $\eta_{1,5}$};
			\node (c3) at (7.0,2.5) {\footnotesize $\eta_{3,3}$};
			\node (a1) at (9.5,2.5) {\footnotesize $\eta_{1,1}$};		
			\node (a4) at (-0.5,5) {\footnotesize $\eta_{1,4}$};
			\node (a2) at (2.0,5) {\footnotesize $\eta_{1,2}$};
			\node (c5) at (4.5,5) {\footnotesize $\eta_{3,5}$};
			\node (b3) at (7.0,5) {\footnotesize $\eta_{2,3}$};
			\node (c1) at (9.5,5) {\footnotesize $\eta_{3,1}$};
		\end{scope}
	
	\begin{scope}[>={Stealth[black]},
		every node/.style={fill=white,circle},
		every edge/.style={draw=red,very thick}]
		%%% Layer 1
		% From d5
		\path [<->] (d5) edge node {\footnotesize UE$_1$} (b4);
		\path [<->] (d5) edge node {\footnotesize  UE$_2$} (c4);
		\path [<->] (d5) edge node {\footnotesize  UE$_3$} (a4);
		
		%%% Layer 2
		% From b4
		\path [<-] (b4) edge node {\footnotesize  UE$_3$} (b2);
		\path [->] (b2) edge node {\footnotesize  UE$_3$} 
		(a5);
		
		% From c4
		\path [<-] (c4) edge node {\footnotesize  UE$_1$} (c2);
		\path [->] (c2) edge node {\footnotesize  UE$_1$}
		(b5);
		
		% From c4
		\path [<-] (a4) edge node {\footnotesize  UE$_2$} (a2);
		\path [->] (a2) edge node {\footnotesize  UE$_2$}
		(c5);
		
		%%% Layer 3
		% From a5
		\path [<-] (a5) edge node {\footnotesize  UE$_2$} (c3);
		\path [->] (c3) edge node {\footnotesize  UE$_2$} 
		(a1);
		
		% From b5
		\path [<-] (b5) edge node {\footnotesize  UE$_3$} (a3);
		\path [->] (a3) edge node {\footnotesize  UE$_3$} 
		(b1);
		
		% From c5
		\path [<-] (c5) edge node {\footnotesize  UE$_1$} (b3);
		\path [->] (b3) edge node {\footnotesize  UE$_1$} 
		(c1);

		
	\end{scope}
}

\newcommand{\PlotMMuRegions}[0]{
	\begin{axis}[
		axis x line=bottom, axis y line=left,
		ymin=1, ymax=8, ytick={1}, extra y ticks={2,5}, ylabel={$M$},
		xmin=0, xmax=1.05, xtick={0,0.4, 1}, xlabel=$\mu$,
		xticklabels={\footnotesize $0$, \footnotesize $\nicefrac{K}{(2K+1)}=\nicefrac{2}{5}$,$1$},
		yticklabels={\footnotesize $1$}, extra y tick labels={\footnotesize $\quad K=2$,\footnotesize $2K+1=5$}, extra y tick style={y tick label style={rotate=90}},
		]
		
		\addplot[name path=f1, very thick, dashed, blue, domain=0:1, smooth]{2};
		
		\path[name path=axis] (axis cs:1,2) -- (axis cs:1,0) -- (axis cs:0,0);
		\addplot[pattern=north west lines, pattern color=OliveGreen] fill between[of=axis and f1];

		\addplot+[name path=f2, no markers, decoration={
		text={}, raise=1ex,
		text align={center}
		}, postaction={decorate}, dashed, very thick, blue, domain=0.4:1, smooth]{2/x};
		
%		\addplot[name path=f3, very thick, dashed, blue, domain=0.4:1, smooth]{5};

		\addplot[name path=f3, very thick, dashed, blue, domain=0.4:0.4375, smooth]{1/(1-2*x)};
		
		\path[name path=yc] (axis cs:0.4375,8) -- (axis cs:1,8);
		
		\path[name path=xc] (axis cs:1,2) -- (axis cs:1,8);
		
		\addplot[pattern=north west lines, pattern color=magenta!55] fill between[of=f2 and yc];
		
		\addplot+[name path=f4, no markers, decoration={
		text={}, raise=1ex,
		text align={center}
		}, postaction={decorate}, dashed, very thick, blue, domain=0.25:0.4, smooth]{2/x};
		
%		\path[name path=axis2] (axis cs:1,8) -- (axis cs:0.25,8) -- (axis cs:0.4,5) -- (axis cs:1,5) -- (axis cs:1,8);

		\path[name path=yc1] (axis cs:0.25,8) -- (axis cs:0.4375,8);
				
		\addplot[pattern=north west lines, pattern color=black!50] fill between[of=f4 and yc1];
		
		\addplot+[name path=f5, no markers, decoration={
		text={}, raise=1ex,
		text align={center}
		}, postaction={decorate}, dashed, very thick, blue, domain=0.02:0.4, smooth]{2/(2*(1-x))+sqrt(4/(4*(1-x)^(2))+2/(x*(1-x)))};
		
%		\addplot+[name path=f6, no markers, decoration={
%		text={}, raise=1ex,
%		text align={center}
%		}, postaction={decorate}, dashed, very thick, blue, domain=0.02:0.4, smooth]{2/(2*(1-x))-sqrt(4/(4*(1-x)^(2))+2/(x*(1-x)))};

		\addplot[pattern=north west lines, pattern color=cyan!90] fill between[of=f4 and f5];
		
		\foreach \M in {1,2,...,8}{
			\foreach \k in {1,..., \M}{ 
				\addplot[red, mark=otimes*, only marks] coordinates {({\k/\M},{\M})};
			}
		}
		
		\node[anchor=west, scale=0.9] at (axis cs: 0.65,4.5) {\textbf{Region A}};
		\node[anchor=west, rotate=-80, scale=0.9] at (axis cs: 0.335,7.95) {\textbf{Region B}};
		\node[scale=0.9] at (axis cs: 0.5,1.5) {\textbf{Region C}};
		\node[rotate=-60, scale=0.9] at (axis cs: 0.15,3.5) {\textbf{Region D}};
		\node[rotate=-65, scale=0.9] at (axis cs: 0.225,6.5) {\textbf{Region E}};
	\end{axis}
}
